Independent low-rank matrix analysis based on the Sinkhorn divergence source model for blind source separation

The so-called independent low-rank matrix analysis (ILRMA) has demonstrated a great potential for dealing with the problem of determined blind source separation (BSS) for audio and speech signals. This method assumes that the spectra from different frequency bands are independent and the spectral coefficients in any frequency band are Gaussian distributed. The Itakura-Saito divergence is then employed to estimate the source model related parameters. In reality, however, the spectral coefficients from different frequency bands may be dependent, which is not considered in the existing ILRMA algorithm. This paper presents an improved version of ILRMA, which considers the dependency between the spectral coefficients from different frequency bands. The Sinkhorn divergence is then exploited to optimize the source model parameters. As a result of using the cross-band information, the BSS performance is improved. But the number of parameters to be estimated also increases significantly, and so is the computational complexity. To reduce the algorithm complexity, we apply the Kronecker product to decompose the modeling matrix into the product of a number of matrices of much smaller dimensionality. An efficient algorithm is then developed to implement the Sinkhorn divergence based BSS algorithm and the complexity is reduced by an order of magnitude.

==> SECTION5.tex <==
\section{SIMULATIONS}

We used some speech signals from the Wall Street Journal (WSJ0) corpus \cite{ref21} as the clean speech source signals and configured test condition followed the SISEC challenge \cite{ref23} with $M=N=2$, where the room size is $8 \times 8 \times 3$ m. The two sources are assumed to be $2$ m away from the center of the two microphones and the microphone spacing is $5.66$ cm. The incident angles of two speakers are randomly selected from $[0^{\circ},90^{\circ}]$ and $[0^{\circ},-90^{\circ}]$ respectively per mixture, where we define the normal direction of the two microphones is $0^{\circ}$. The image source model \cite{ref25} is used to generate the room impulse responses, where the sound absorption coefficients are calculated by Sabine's Formula \cite{ref26} under the room shape described and reverberation time $T_{60}$ selected from $[0,600]$ ms with an interval of $50$ ms. For each gender combination and each $T_{60}$, we generate $100$ mixtures for evaluation. The sampling rate is set to $16$ kHz.


The parameters $\mu$ and $\gamma$ of SDILRMA were set to $100$, and $10$, respectively. We compared SDILRMA with AuxIVA \cite{ref8}, MNMF \cite{ref22}, ILRMA \cite{ref5}, $t$-ILRMA and sGD-ILRMA \cite{ref20}. The performance metric used is the signal-to-distortion ration (SDR) and source-to-interferences ratio (SIR) \cite{ref24}.
\begin{figure*}[t]
\centering
\vspace{-0.7cm} %调整图片与上文的垂直距离
\subfloat[female+female]{\includegraphics[width=1.85in]{SDRimp_RC1FF.eps}%
\label{fig_SISEC2011_5a}}
\hfil
\subfloat[female+male ]{\includegraphics[width=1.85in]{SDRimp_RC1FM.eps}%
\label{fig_SISEC2011_5b}}
\hfil
\subfloat[male+male ]{\includegraphics[width=1.85in]{SDRimp_RC1MM.eps}%
\label{fig_SISEC2011_5c}}
\hfil
\subfloat[female+female ]{\includegraphics[width=1.85in]{DSIRimp_RC1FF.eps}%
\label{fig_SISEC2011_5d}}
\hfil
\subfloat[female+male ]{\includegraphics[width=1.85in]{DSIRimp_RC1FM.eps}%
\label{fig_SISEC2011_5e}}
\hfil
\subfloat[male+male ]{\includegraphics[width=1.85in]{DSIRimp_RC1MM.eps}%
\label{fig_SISEC2011_5f}}
\vspace{-0.2cm}
\caption{SDR improvement and SIR improvement of the comparison methods on WSJ0-reverb.}
\label{Fig2}
\vspace{-0.5cm}
\end{figure*}

Fig. \ref{Fig2} presents the results on speech separation with respect to the average SDR and SIR improvements. It is seen that SDILRMA outperforms MNMF, ILRMA and their extensions $t$-ILRMA and sGD-ILRMA under anechoic conditions, which demonstrates the effective of the Sinkhorn divergence for source model related parameters.
\begin{figure}[t]\label{Fig3}
\vspace{-0.5cm}
\begin{minipage}[b]{1\linewidth}
  \centering
  \centerline{\includegraphics[width=15cm]{Spectra.pdf}}
%  \vspace{2.0cm}
%  \centerline{(a) Result 1}\medskip
\end{minipage}
\vspace{-0.7cm}
\caption{ The separated spectrogram from two speakers in condition 1. The right one is the original two sources, The middle is the separated results from ILRMA, and the left is the results of SDILRMA.}
\label{Fig3}
\vspace{-0.5cm}
\end{figure}
Fig. \ref{Fig3} shows the original spectrogram of two speakers and its estimated separated signals by ILRMA and SDILRMA. The figure shows that ILRMA and SDILRMA are effective, but sometimes, the permutation problem in subband may happen in ILRMA, the Sinkhorn divergence-based source model will give a more robust results. 
